Learning from Limited and Imperfect Data

The distribution of data in the world (eg, internet, etc.) significantly differs from the well-curated datasets and is often over-populated with samples from common categories. The algorithms designed for well-curated datasets perform suboptimally when used for learning from imperfect datasets with long-tailed imbalances and distribution shifts. To expand the use of deep models, it is essential to overcome the labor-intensive curation process by developing robust algorithms that can learn from diverse, real-world data distributions. Toward this goal, we develop practical algorithms for Deep Neural Networks which can learn from limited and imperfect data present in the real world. This thesis is divided into four segments, each covering a scenario of learning from limited or imperfect data. The first part of the thesis focuses on Learning Generative Models from Long-Tail Data, where we mitigate the mode-collapse and enable diverse aesthetic image generations for tail (minority) classes. In the second part, we enable effective generalization on tail classes through Inductive Regularization schemes, which allow tail classes to generalize as effectively as the head classes without requiring explicit generation of images. In the third part, we develop algorithms for Optimizing Relevant Metrics for learning from long-tailed data with limited annotation (semi-supervised), followed by the fourth part, which focuses on the Efficient Domain Adaptation of the model to various domains with very few to zero labeled samples.

==> ignore.tex <==

Deep Neural Networks achieve near-human performance on several benchmark datasets, yet they are not as robust as the human visual system. Their success relies on the proximity of test samples to the distribution of training data, resulting in unexpected behavior when encountered with even minor distribution shifts during inference. Deep Networks are also known to be susceptible to adversarial attacks, which are crafted imperceptible perturbations to their inputs, that can lead a classification model to confidently misclassify images into unrelated classes. The rapid adoption of Deep Networks in several critical applications makes it imperative to understand these failure models and develop reliable risk mitigation strategies. This thesis focuses on developing efficient and effective methods for improving the robustness of Deep Networks to both adversarial attacks and distribution shifts. The thesis is organized into four parts. 

State-of-the-art adversarial defenses use multi-step adversarial training, where the training data is augmented with adversarially perturbed images that are typically generated using ten steps of optimization, incurring additional computational cost during training. In the first part of the thesis, we develop \textbf{Efficient Adversarial Defenses} to overcome the large computational overhead of existing adversarial training methods. 
 
While Adversarial Training improves the robustness of Deep Networks significantly, one of the key challenges that limits its practical use is the associated drop in natural or clean accuracy, referred to as the robustness-accuracy trade-off. In the second part of the thesis, we propose methods for \textbf{Improving the Effectiveness of Adversarial Training} by mitigating various challenges that limit their performance and utility. 

Instance-discrimination based Self-Supervised Learning (SSL) methods have shown success in learning transferable representations without using labeled training data. However, these methods are more computationally expensive than supervised training. Moreover, self-supervised adversarial training 
In the third part, we propose efficient and effective algorithms for \textbf{Self-Supervised Learning of Robust Representations}. 

Finally, we propose methods for \textbf{Improving Robustness to Distribution Shifts in Data}.

\textbf{Efficient Adversarial Defenses}: State-of-the-art adversarial defenses use multi-step adversarial training, where the training data is augmented with adversarially perturbed images that are typically generated using ten steps of optimization, incurring additional computational cost during training. To overcome this computational overhead, we first propose \emph{Bit Plane Feature Consistency Regularizer (BPFC)} to achieve robustness without the generation of adversarial attacks during training by imposing consistency on the representations of differently quantized images.
We further develop methods for improving robustness while maintaining a low computational cost by using single-step adversarial attacks for training. Single-step adversarial training is known to converge to a degenerate solution with sub-optimal robustness due to the obfuscation of gradients at the data samples, which leads to the generation of weaker attacks during training. To mitigate this, we propose \emph{Guided Adversarial Training (GAT)} and \emph{Nuclear Norm Adversarial Training (NuAT)} that explicitly enforce function smoothing in the vicinity of each data sample, thereby preventing obfuscated gradients and resulting in improvements over existing single-step defenses and several multi-step defenses as well. 


\textbf{Improving the Effectiveness of Adversarial Training:} While Adversarial Training improves the robustness of Deep Networks significantly, one of the key challenges that limits its practical use is the associated drop in natural or clean accuracy, referred to as the robustness-accuracy trade-off. 
To address this, we first propose \emph{Feature Level Stochastic Smoothing (FLSS)} based classifier, which introduces stochasticity in the network predictions, and utilizes the same for smoothing decision boundaries and rejecting low confidence predictions, thereby boosting the robustness and clean accuracy of the accepted samples. We further investigate the reasons for a higher robustness-accuracy trade-off at larger perturbation bounds where some attacks change the perception of a human or an Oracle, while other attacks do not. The proposed \emph{Oracle-Aligned Adversarial Training (OAAT)} overcomes this trade-off by introducing specific attack and defense losses for Oracle-Sensitive and Oracle-Invariant adversarial examples.
While robustness-accuracy trade-off can be alleviated using more diverse data for training, complex data augmentations have not been successful with Adversarial Training. We investigate the reasons for this, and propose \emph{Diverse Augmentation based Joint Adversarial Training (DAJAT)} that addresses the same by using separate batch-normalization layers for simple and complex augmentations and a Jensen-Shannon divergence loss to encourage their joint learning.



\textbf{Self-Supervised Learning of Robust Representations:} Instance-discrimination based Self-Supervised Learning (SSL) methods have shown success in learning transferable representations without using labeled training data. However, these methods are more computationally expensive than supervised training. We investigate the reasons for their slow convergence, and propose to improve the same by combining them with pretext tasks such as rotation prediction, which reduce the noise in the training objective. We further utilize these pretrained SSL models in a teacher-student setting for training adversarially robust models without labels. We propose \emph{Projected Feature Adversarial Training (ProFeAT)}, where the pretrained SSL projector of the teacher is utilized in order to obtain significant gains in clean accuracy of the adversarially trained student. The proposed attack loss coupled with the use of strong data augmentations leads to significantly better robustness-accuracy trade-off when compared to prior works. 

\textbf{Improving Robustness to Distribution Shifts in Data:} Deep Neural Networks are known to be brittle to even minor distribution shifts during inference. We put forth the (simple) \emph{Feature Replication Hypothesis} to explain this behaviour, and propose the \emph{Feature Reconstruction Regularizer (FRR)} to overcome this brittleness by ensuring that the learned features can be reconstructed back from the logits, thereby encouraging the use of more diverse features for classification. We further propose \emph{Diversify-Aggregate-Repeat Training (DART)} that trains diverse models using different augmentations (or domains) to explore the loss basin, and further Aggregates their weights repeatedly over training to combine their expertise and obtain improved generalization. We finally aim to utilize the  superior generalization of black-box Vision-Language Models (VLMs) for better OOD generalization in vision tasks. We propose \emph{Vision-Language to Vision - Align, Distill, Predict (VL2V-ADiP)}, a teacher-student setting which first aligns and then distills  the representations of the teacher to the pretrained student.

